Breaking On-Chip Communication Anonymity using Flow Correlation Attacks

Network-on-Chip (NoC) is widely used to facilitate communication between components in sophisticated System-on-Chip (SoC) designs. Security of the on-chip communication is crucial because exploiting any vulnerability in shared NoC would be a goldmine for an attacker that puts the entire computing infrastructure at risk. We investigate the security strength of existing anonymous routing protocols in NoC architectures, making two pivotal contributions. Firstly, we develop and perform a machine learning (ML)-based flow correlation attack on existing anonymous routing techniques in Network-on-Chip (NoC) systems, revealing that they provide only packet-level anonymity. Secondly, we propose a novel, lightweight anonymous routing protocol featuring outbound traffic tunneling and traffic obfuscation. This protocol is designed to provide robust defense against ML-based flow correlation attacks, ensuring both packet-level and flow-level anonymity. Experimental evaluation using both real and synthetic traffic demonstrates that our proposed attack successfully deanonymizes state-of-the-art anonymous routing in NoC architectures with high accuracy (up to 99%) for diverse traffic patterns. It also reveals that our lightweight anonymous routing protocol can defend against ML-based attacks with minor hardware and performance overhead.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> section/Comments.tex <==
\newpage

\section{Responses to Reviewer Comments}
We would like to thank the reviewers for their thorough and insightful comments. We have modified the manuscript to address various issues raised by the reviewers. This section outlines all the reviewer comments and our responses in terms of how we have addressed the issues in the modified manuscript. The modifications are marked in blue in the manuscript. 

% \vspace{4mm}
\subsection{REVIEWER 1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent \textbf{Comment 1:} The recall value of 80.28\% for the 16×16 mesh size (Table 7) and the precision value of 87.15\% for the noise level p = 80 (Table 8) indicate a sharp drop in performance compared to the prior size and noise-level. These edge case results may indicate the limits of the model's effectiveness and practicality in real-world scenarios. The authors should address the implication of these results.

\color{blue}

\vspace{3mm}
\noindent \textbf{Response:}  Thank you for the comment. The drop in recall observed with the 16x16 mesh size in Table 7, as compared to the 8x8 configuration, can largely be attributed to the significant scaling up of the network on chip. The 16x16 mesh has four times as many nodes and approximately double the average number of hops (10.67 compared to 5.33 for the 8x8 mesh), introducing more indirect noise such as queuing delays that impact communication pattern observed through inter-flit delays. 
%This non-linear scaling intensifies the complexity and noise within the system, naturally leading to lower performance metrics. 
It is important to note that the observed recall of 80\% is still high enough to mount a successful attack or disrupt privacy as discussed in Section 3.1. 
%This significantly enhances the adversarial capability to launch attacks within such a large network configuration. Considering potential improvements, a deeper DNN model, adhering to the principles discussed in our model selection methodology (Section~\ref{subsec:dnn-arc}), might slightly enhance performance in handling the complexities associated with larger mesh sizes.

While we notice a sharp drop in precision at higher noise levels, the recall still remains robust at around 98\% (Table 8). Recall is the most important metric from an adversarial perspective, as detailed in Section 5.3 and in response to Comment 2. 
While lower precision may lead to resources being spent on false positives, this concern is minor compared to the potential damage from high recall rates. 
The proposed attack is applicable in real-world scenarios since 8x8 and 16x16 cover many real-world NoC architectures. For example, Intel's Xeon® Scalable Processor~\cite{Intelxeon} supports up to 64 cores, which is comparable to an 8x8 configuration. 
%This suggests that despite the noted declines in certain metrics under edge conditions, the overall utility and robustness of our approach in real-world scenarios remain substantial.  
We have included this discussion in Section 5.5 and 5.6.





% To conclude, the model exhibits strong potential in operational environments, particularly in recognizing and mitigating threats effectively despite the complexities introduced by scale and noise.

% \begin{itemize}
%     \item If we focus on increasing mesh size results, 16x16 is 4 times nodes as 8x8.
%     \item 8x8 mesh have 5.33 average hops while 16x16 has 10.67 (2x times).
%     \item because of this non-linear scaling up, there is relatively more indirect noise (queuing delays, e.t.c) affecting the 16x16 communication results in low performance metrics.
%     \item Still when we compare it with the baseline of random prediction, which will have 50\%, 80\% recall is significantly higher and can give strong advantage to the adversary.
%     \item A deeper DNN model that sticking to fundamentals discussed in model selection~\ref{subsec:dnn-arc} could be able to perform slightly better for increasing mesh size, which can better learn these noises.
%     \item For current NoC-based MPSoC with around 64 processors, for example  Intel's Xeon® Scalable Processor~\cite{Intelxeon} supports up to 60 cores, the proposed attacks performs well.


%     \item If we focus on the increasing noise, even though there is a sharp drop in precision the recall doesn't see a drop (it stays around 98\%).
%     \item As discussed in Section~\ref{sec:ex-train-test} and Comment 2, recall stays as the most critical metric when consider in perspective of the attacker.
%     \item The drop in precision of the correlation traffic detection will results in attacker spending resources on false positives but it is negligible compared to harm attacker can done because of having high recall value.

%     \item To conclude ... (TODO-: write a one sentence positive conclusion to the comment)
    
    




%     % \item Intel's Xeon® Scalable Processor~\cite{Intelxeon} supports up to 60 cores.
    
% \end{itemize}


\vspace{4mm}
\color{black}

\noindent \textbf{Comment 2:} The discussion of the evaluation ML-based attack could address the implication of incorrect labelling by the ML-based attack.

\color{blue}

\vspace{3mm}
\noindent \textbf{Response:}  Thank you for the comment. Incorrect labeling by the ML based attack (misclassifications ) can have significant implications, and it is important to consider them from the perspective of an attacker. Misclassifications can be divided into two types: false positives and false negatives. False positives occur when uncorrelated traffic is incorrectly identified as correlated. In this scenario, an adversary would allocate resources to act upon these false leads to launch further attacks, ultimately yielding no actual threat. While pursuing false leads might seem inefficient, adversaries usually have sufficient resources and can inflict significant damage when they correctly identify correlated nodes. This potential for harm outweighs the minor setbacks caused by occasional false positives. On the other hand, false negatives represent a critical error from the attackers standpoint. This type of error occurs when actual correlated communicating pair go undetected. Missing such opportunities can be detrimental to the adversary’s objectives, particularly if the goal is to cause maximum disruption. Recall, which measures the model's ability to identify all correlated traffic pairs, is arguably more critical than precision in this context, as high recall minimizes false negatives, ensuring fewer correlated pairs go unnoticed. This aligning with an adversary’s aim to identify and exploit every traffic correlation. We have included this discussion in Section 5.6.






% If we consider false positives, where a uncorrelated traffic is considered correlated. The adversary will spend it's resources on launching further attacks on top of the prediction and eventually gaining nothing. If we consider False Negatives adversaries will disregard this and miss chances in launching actual attacks.  In terms of adversary False Positives is fine because normally they will have more resources and in terms of False Negatives they will miss the chance for an successful attack, since adversaries aim is to disturb the system at maximum. Therefore, in terms of attackers Recall which measures the ability of a model to find all positives, is more important than precision.

\vspace{4mm}
\color{black}

\subsection{REVIEWER 2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Comment 1:} The paper has a few limitations, including ``The paper discusses training the ML model only once in the lifetime of SoC as detecting correlation can be computationally expensive.''

\color{blue}

\vspace{2mm}
\noindent \textbf{Response:}  Thank you for the comment. The expression ``once in the lifetime of the SoC'' unintentionally suggested a more rigid approach than intended. To clarify, while the initial training of the ML model is computationally intensive, we do not limit retraining to only once during the SoC's lifetime, but can be retrained periodically as needed. This allows for adaptation to new applications and traffic patterns throughout the lifetime of the SoC. We have rephrased the sentence to avoid the confusion: ``While training the ML model for detecting correlation can be computationally expensive, it is not a limiting factor since the training is a one-time activity. Note that the model can be retrained, if needed after specific intervals, to ensure that it remains effective and up-to-date throughout its operational lifetime.''


% \begin{itemize}
%     \item Not throughout lifetimebut not each time
%     \item can train iterativel ytunning for new application and other changes in system
%     \item 
% \end{itemize}


\vspace{3mm}
\color{black}


\noindent \textbf{Comment 2:} The paper doesn’t discuss the interface between PyTorch and gem5 to train the DNN.

\color{blue}

\vspace{2mm}
\noindent \textbf{Response:}  Thank you for the comment. The training of the DNN has three major phases: data collection (gem5), data preprocessing, training and validation (PyTorch). We automated data collection using the gem5 simulator with a shell script that simulates different benchmarks and application mappings. This process output traffic traces from gem5 as textual logs.
We implemented a Python script to preprocesses these traffic traces to generate inter-flit delay arrays represented as 2D numpy arrays. This preprocessed data was used to train and validate the DNN model implemented in PyTorch. We have included these details in Section 5.1.


% \begin{itemize}
%     \item Data for training collected via multiple iterations running gem5 simulator by changing the benchmarks, application mapping.
%     \item Collecting data from gem5 is automated through script for different benchmark and mapping. 
%     \item We will get the network traces from gem5 as logs with textual information.
%     \item Then preprocessing of the data to suite the ml model input as numpy array is automated through an python script which parse these logs and generate inter-flit arrays as discussed in Section~\ref{sec:attack}.
%     \item This collected data is used to train and validate model in training phase.
% \end{itemize}

\vspace{3mm}
\color{black}


\noindent \textbf{Comment 3:} The paper has a few limitations, including, ``An epoch size of 10 and 20 seems to be small for the convergence of a DNN model."

\color{blue}

\vspace{2mm}
\noindent \textbf{Response:}  Thank you for the comment. The optimal number of epochs for model convergence can vary widely depending on specific task parameters, data characteristics, model architecture, and training methodologies. Our decision to limit training to 10-20 epochs was primarily based on initial experiments with early stopping, which halts training when validation error ceases to decrease. This approach consistently showed that performance stabilized within this range. Additionally, restricting the number of epochs to 10-20 served as a regularization technique to further mitigate the risk of overfitting. It is important to note that our proposed DNN model is very simple (7 layers). Therefore, shorter training cycle (10-20 epochs) allows for effective learning without the risk of overfitting. We have included these details in Section 5.2.

% \begin{itemize}
%     \item The effective epoch size for training a Deep Neural Network (DNN) model can vary widely based on several factors related to the specific task, data characteristics, model architecture, and training methodology.
%     \item The rational and experimental steps to sticking to epoch size of 10-20 as follows.
%     \item Initial experiments with early stopping based on validation error suggested to use between 10 to 20. 
%     \item To avoid overfitting we stick with 10 - 20 epochs.
%     \item The main reason for this is because model is relatively simple (have 7 layers) compared to large models such as ResNet-50 that have 50 layers.
% \end{itemize}


\vspace{3mm}
\color{black}


\noindent \textbf{Comment 4:} The paper discusses only a few related works on NoC security.

\color{blue}

\vspace{2mm}
\noindent \textbf{Response:} We have updated Section 2.3 with more related work on NoC security.


\vspace{3mm}
\color{black}



\noindent \textbf{Comment 5:} This statement is not fully correct as NoC is used significantly for data traffic: “Traffic characteristics of NoC and traditional networks are significantly different because NoC uses its traffic primarily for cache coherence messages.”

\color{blue}

\vspace{2mm}
\noindent \textbf{Response:} Thank you for your comment. We have rephrased the sentence as: “Traffic characteristics differ significantly between NoC and traditional network due to varying use cases. NoC is used for routing simple on-chip communication traffic, such as cache coherence, memory accesses, and inter-processor communications. In contrast, traditional networks handle complex use cases, such as enterprise data services, cloud computing tasks, and multimedia streaming.”

\vspace{3mm}
\color{black}




